Continuously Managing NFRs: Opportunities and Challenges in Practice

Non-functional requirements (NFR), which include performance, availability, and maintainability, are vitally important to overall software quality. However, research has shown NFRs are, in practice, poorly defined and difficult to verify. Continuous software engineering practices, which extend agile practices, emphasize fast paced, automated, and rapid release of software that poses additional challenges to handling NFRs. In this multi-case study we empirically investigated how three organizations, for which NFRs are paramount to their business survival, manage NFRs in their continuous practices. We describe four practices these companies use to manage NFRs, such as offloading NFRs to cloud providers or the use of metrics and continuous monitoring, both of which enable almost real-time feedback on managing the NFRs. However, managing NFRs comes at a cost as we also identified a number of challenges these organizations face while managing NFRs in their continuous software engineering practices. For example, the organizations in our study were able to realize an NFR by strategically and heavily investing in configuration management and infrastructure as code, in order to offload the responsibility of NFRs; however, this offloading implied potential loss of control. Our discussion and key research implications show the opportunities, trade-offs, and importance of the unique give-and-take relationship between continuous software engineering and NFRs. Research artifacts may be found at https://doi.org/10.5281/zenodo.3376342.

==> 05a_results_practices.tex <==
% then add a sentence summarizing the NFR concerns that each organization seems to have had.
% and a general trend, i.e. CM most important for two of them (explain a bit), whereas the top three
% Alpha: security, scalability, perforamance -- put it in the context of its product/operations
% Beta: Usability, performance and reliability
% Gamma: performance, reproducibility, scalability

%===============================================================================
\section{Study Findings} \label{findings}

In this section we describe the themes (practices and challenges) we identified in these three organizations' handling of NFRs in their continuous practice. We summarize these practices and challenges in Table \ref{tab:findings}. 

\begin{table}[htb]%[thb]
\caption{Summary Practices and Challenges of small agile organizations handling NFRs with continuous practices}
\label{tab:findings}
    \begin{tabular}{cl}
    \toprule
    \multirow{4}{*}{Practices}& Put a number on the NFR \\
    & Let someone else manage the NFR \\
    & Write your own tool to check the NFR \\
    & Put the NFR in source control \\
    \midrule
    \multirow{3}{*}{Challenges}& Not all NFRs are easy to automate \\
    & Functional requirements get prioritized over NFRs \\
    & Lack of shared understanding of an NFR \\
    \bottomrule
    \end{tabular}
\end{table}
%===============================================================================

All three software organizations in our study care deeply about non-functional requirements in their software development. 
Alpha, in the data crowdsourcing business, is most concerned about \nfr{configuration management}, \nfr{security}, and \nfr{scalability}. These three NFRs are vital to Alpha's business as Alpha processes and stores data from large numbers of users per day on a third party hosted infrastructure.
Beta, a leading e-commerce platform, is primarily concerned with \nfr{usability}, \nfr{performance}, and \nfr{stability/reliability}, as their applications handle millions of user commercial transactions per day.
Finally, Gamma, an online advertisement content provider, requires \nfr{performance}, \nfr{revenue}, and \nfr{configuration management} to ensure that Gamma's infrastructure can effectively deliver Gamma's content to Gamma's wide audience.

Table \ref{tab:nfr-ranking} shows the overall ranking and individual ranking for each organization based on the frequency that the code representing the NFR appeared in our data (with at least 30 occurrences). Gamma's number 2 ranking (revenue) is notably absent from the table due to less than 30 overall occurrences, despite the high number of occurrences at Gamma.

%Our findings describe existing practices found at our subject organizations, and the NFR challenges they are facing.


Throughout our reporting (and in Table \ref{tab:nfr-ranking}), we ensure that we link our codes or particular findings to the evidence (interview text) as much as possible using quotes as well as spark-histograms. 
First introduced by Ying and Robillard \cite{Ying2014}, these histograms are intended as a compact and quick form of assessment of our findings: each histogram captures the 18 participants interviewed on the x-axis, while the y-axis shows the number of times the given code was mentioned by each participant, relative to the total number of mentions of that code. We also show the total number of mentions following the histogram.

The x-axis is ordered to match Table \ref{tab:participant-information}. 
For example, consider the histogram for our code \nfr{configuration management} \histno{ConfigurationManagementNFR}{103}, which shows participants 3-6 mentioned this code more often than the other participants, and across all transcripts, this code occurred 103 times.  

%===============================================================================
\begin{table}%[h]
\caption{Ranking of NFRs by frequency of mention. Sorted by overall frequency. Columns Alpha, Beta, \& Gamma refer to rank within each organization. (T indicates a tie)}
\label{tab:nfr-ranking}
\begin{threeparttable}
\begin{tabular}{rlcrrr}
\toprule
\textbf{Rank} & \textbf{NFR} & \textbf{Histo.} & \textbf{Alpha} & \textbf{Beta} & \textbf{Gamma} \\ \midrule 
1 & Config. Mgmt. & \histogram{histogram/ConfigurationManagementNFR.tex} & 1 & \tied{12} & 3 \\
2 & Performance & \histogram{histogram/PerformanceNFR.tex} & \tied{4} & 2 & 1 \\
3 & Security & \histogram{histogram/SecurityNFR.tex} & 2 & \tied{5} & 6 \\
4 & Scalability & \histogram{histogram/ScalabilityNFR.tex} & 3 & \tied{5} & 5 \\
5 & Usability & \histogram{histogram/UsabilityNFR.tex} & \tied{14} & 1 & \tied{9} \\
6 & Reproducibility & \histogram{histogram/ReproducibilityNFR.tex} & \tied{4} & \tied{5} & 4 \\
7 & Testability & \histogram{histogram/TestabilityNFR.tex} & \tied{6} & 4 & 8 \\
8 & Stab./Reli. & \histogram{histogram/StabilityReliabilityNFR.tex} & 10 & 3 & \tied{9} \\
9 & Availability & \histogram{histogram/AvailabilityNFR.tex} & \tied{6} & \tied{5} & \tied{12} \\
10 & Maintainability & \histogram{histogram/MaintainabilityNFR.tex} & 8 & \tied{5} & \tied{17} \\
11 & Readability & \histogram{histogram/ReadabilityNFR.tex} & 9 & \tied{15} & \tied{14} \\
\bottomrule
\end{tabular}
%\begin{tablenotes}\footnotesize
%\item[*] T indicates a tie.
%\item[] \-bility
%\end{tablenotes}
\end{threeparttable}
\end{table}
%===============================================================================

%===============================================================================
\subsection{Practices For Handling NFRs in a continuous context}
%===============================================================================
Our first research question examines how NFRs are managed within each organization---the strategies and practices they use to handle NFRs in the context of small, agile teams following a set of continuous practices. 
We identified four strategies from our interviews. 
These were to: Put a number on the NFR, Let someone else manage the NFR, Write your own tool to check the NFR, and Put the NFR in source control. We discuss each strategy in turn. 

%\todo{For each discussion point, Make sure we add more context with respect to the organization's product, ie Gamma is advertising, etc. 1.) quote, 2.) person, 3.) nfr 4.) role 5.) business goal}


%===============================================================================
\subsubsection{Put a Number on the NFR}
\label{sec:res_metrics}
%===============================================================================
The first strategy for dealing with NFRs is establishing metrics and measurements to help validate and assess a particular NFR once the NFR is treated.
The concept of measuring an NFR was frequently discussed during our interviews \hist{Metrics}{154}.
When an organization tracks pertinent measurements for NFRs, measurement indicators calculated by the organization's deployment pipeline provide valuable insight on NFRs.
For Gamma, these include \nfr{performance} and \nfr{availability}: \q{a lot of the [caching ratio] that we have from <redacted> with our CDN or caching provider goes up there because that's usually a pretty good indication that something has gone wrong. It also drastically affects \nfr{performance}} (P14).
However, Gamma could also evaluate \nfr{performance} NFRs with the addition of other metrics: \q{Some of the metrics [we use], for example revenue or [number of users] a specific page has had [...], might be able to infer \nfr{performance} of the website basically based on how many users they thought versus [how many actually used the page]} (P18). 
For Gamma, \nfr{performance} and \nfr{availability} are important aspects of the organization's business.
Since Gamma's \nfr{revenue} is driven by advertisements, a failure to load their application or a ``laggy" application experience would drive users away. Hence, \nfr{performance} ranks first and \nfr{availability} ranks seventh by frequency for Gamma as shown by Table \ref{tab:nfr-ranking}.

Alpha collects data from millions of users worldwide. 
If response times drop below a specific measurement, the drop signifies a likely \nfr{performance} decline, which may impact a significant number of users and hurt Alpha's crowdsourcing business. 
As a result, defining quantifiable measures is necessary: \q{We could have a certain amount of monitoring set up [...] You're also defining which alarms are set. Therefore, if requests [drop] below <redacted> milliseconds and that's what you want to hold it to. Then that would be codified in the alarm} (P5).
Without setting a quantitative measure, Alpha may not receive warning that its software experienced a dramatic drop in \nfr{performance}. 
Similarly, Beta provides a platform for many stores and \nfr{usability} is important for those stores; tracking the number of customer actions to complete a transaction may help measure \nfr{usability}: \q{I can tell you that 90\% of our customers have less than <redacted> items [...] They'll [say] we know that each [order] requires <redacted> page loads} (P7).
By identifying key metrics, an organization may create effective tests for NFRs. 

% We find that these monitoring mechanisms they put in place (typically dashboards that are accessible to developers) provide what most participants refer to as the feedback loop.
A key factor for the success of identifying measurements for NFRs is due to the feedback loop \histno{FeedbackLoop}{46}{}.
The feedback loop is an integral part of any continuous practice and is one of the earliest perceived benefits of adopting a continuous practice.
For Alpha, which deals with a lot of user data, effectively managing \nfr{security} NFRs is important for its business. Hence, the presence of a feedback loop enhanced with automatic notifications regarding infrastructure \nfr{security} positively impacts developer workflow.
%\q{A few things that we've got various forms of monitoring [...] For instance, when people are changing IAM policies not that there's automated feedback on that, but at least people who need to be aware of IAM changes are automatically notified} (P3).
Ideally, an organization has a fast feedback loop so that the organization can quickly pinpoint problematic NFRs or alter an NFR based on customer response. 
As Beta operates an e-commerce platform that serves many stores, it is imperative that the platform is available to customers. A feedback loop provides the ability for Beta to quickly identify bugs that crash the software: \q{I think quick feedback is the core of DevOps so that we will see what broke or will see when [software] breaks quickly} (P6) and \q{By being alerted of things going that aren't working sooner rather than later. It allows us to move much quicker much more quickly and our development and it reduces risk because things are integrated more frequently} (P6).
In particular, the feedback loop is most useful if it is a \emph{quick} feedback loop and many organizations strive to reduce the time required for a feedback loop to complete, e.g. \q{Developers really want [the] feedback loop to be tight} (P13). Although a feedback loop may provide meaningful metrics regardless of the response time of the feedback, a \emph{quick} feedback loop ensures that feedback is up to date with fast moving requirements which coincides with the rapid development cycles used by small, agile organizations. 

%===============================================================================

%===============================================================================
\subsubsection{Let Someone Else Manage the NFR}
%===============================================================================
The most popular approach to managing NFRs we found was to let someone else do it (i.e. offload), where the `someone else' is typically a large cloud services provider \histno{NFROffloading}{155}{}. 
Offloading an NFR means that an organization allows another platform or tool \histno{Tooling}{262}{} 
to manage the NFR on the organization's behalf (which still requires some form of internal configuration).

NFR offloading is a common practice for two reasons. 
One, it means the provider assumes all responsibility for satisfying and achieving the NFR. 
For example, AWS manages nearly all \nfr{availability} concerns, rather than the organization. 
Two, it allows the organization to easily ratchet \cite{bellomo2014} their NFR measures. If more \nfr{performance} is needed, the provider can be asked to expand instances or CPU capacity.
For example, by using a cloud provider, Alpha is able to offload \nfr{availability} and \nfr{scalability} requirements, both of which are critical success factors to their product success. They get world-leading expertise in these NFRs, and essentially (given their current size) limitless scaling.

We show three examples of NFRs that were offloaded. 
The first NFR is \nfr{configuration management}. 
\nfr{Configuration management} is an emerging NFR that refers to the need to ensure the code and associated hardware are in a sound state at any point in time. 
However, many organizations do not manage their own hardware or infrastructure.
Instead, they rely on cloud providers, such as Amazon Web Services (AWS), Microsoft Azure, or Google Cloud, for their infrastructure needs.
Cloud providers are favoured by DevOps engineers as they have access to a cloud provider support team to assist with issues, \q{Cloud providers are awesome. I love being able to just file a support ticket} (P12). 
We also found that the organizations we studied made frequent use of \nfr{configuration management} tooling such as Docker, Terraform, and Kubernetes.
These tools facilitate efficient and repeatable environment creation, e.g. \q{the most important part is that the builds and the environment they run on and deploy to are defined in a repeatable way or state} (P5).

Overall, \nfr{configuration management} was the most referenced specific NFR \histno{ConfigurationManagementNFR}{103}{}. \nfr{Configuration Management} tools also help achieve \nfr{reproducibility} \histno{ReproducibilityNFR}{52}{}.
For example, \nfr{configuration management} helps Beta maintain three separate software stacks.
Beta's \nfr{configuration management} tooling manages dependencies by allowing developers and testers to easily create or re-create an environment and application, e.g. \q{it automatically does it in the Docker compose files. So we've automated a lot of dependency updates and stuff like that} (P11). % \todo{link to business goals}
%and \q{I think some people believe Docker helps extract abstract complexities and difficulties and provides benefits that outweigh, its learning curve and overhead costs} (P1).


% security 
Our second example is \nfr{security} \histno{SecurityNFR}{68}{}, which our study found was also offloaded to a third party service. 
Instead of an organization laboriously maintaining and provisioning \nfr{security} checks on its resources, \nfr{security} and \nfr{privacy} may be intrinsically supported by a third party provider.
Beta maintains an extensive customer database and are keenly interested in \nfr{security} and \nfr{privacy} of the database.
However, management of the \nfr{security} aspects can be offloaded to third party tools, e.g. \q{I believe that's all codified in like the Docker and Kubernetes world} (P6). For instance, Kubernetes can use namespaces to isolate user access control. Other tools can scan for malicious third-party package dependencies.
 
Gamma utilizes a key management system directly from one of the cloud providers, e.g. \q{we use a security Magic Key Management pool from <redacted>} (P16), which frees Gamma developers from having to worry (extensively) about key management issues.

% \nfr{performance} & \nfr{availability} & \nfr{scalability} & stability/reliability
Our final example is for \nfr{performance} \histno{PerformanceNFR}{88}{}, and related NFRs \nfr{availability} \histno{AvailabilityNFR}{39}{}, \nfr{stability/reliability} \histno{StabilityReliabilityNFR}{41}{}, and \nfr{scalability} \histno{ScalabilityNFR}{56}{}.
Cloud providers in particular are heavily used to achieve these NFRs.
For example, Alpha collects a very large amount of data from users spread out across the globe on a daily basis, so having a highly distributed, available, performant, and scalable system is paramount, e.g. \q{everything's running in the cloud. [...] You put your web application up there and it's immediately spread across however many availability zones and nodes as you want} (P5).
% and \q{we are concerned with \nfr{performance} [...] latency, \nfr{scalability}.} (P3)

NFR offloading also provides ratcheting capability for key NFRs. 
All three organizations highlighted their ability to increase the amount of resources they consume from their cloud providers if they hit a particular NFR bottleneck. 
Increasing the amount of resources obviously has financial cost.
These additional resources allow the organization time to properly investigate the source of the bottleneck.
For example, Gamma and Alpha both noted that they can simply pay more to the cloud provider, e.g., 
%\q{something's going burning through too much. We gotta deal with it now versus hey is burning too much and it'll cost a few bucks we can deal with it tomorrow} (P17) and 
\q{We just put money in the machine and made it better} (P5).

%Naturally, to take advantage of the ability to simply increase \nfr{performance}, \nfr{availability}, \nfr{scalability}, stability/reliability an organization must have the foresight and ability to reliably determine the desired levels of service required, which is felicitous within a continuous software life cycle by providing immediate feedback to developers, e.g. \q{Yeah, that's I think I would find that kind of automation that I created that be more of a making developers happy and making the system. Oh, yeah, I guess I was more consistent and reliable you have a bit more confidence that the change you make is whatever absolutely everything} (P18).

%===============================================================================
%\todo{Make sure we add more context with respect to the organization's product, ie Gamma is advertising, etc. 1.) quote, 2.) person, 3.) nfr 4.) role 5.) business goal}

%Continuous practices would not exist without these tools as the \nfr{configuration management} would simply be unsustainable for any one organization to manage on their own.

%For example, \q{we really rely on the cloud provider to handle that aspect. If the feature does not work out for us, then we'll have to consider a second secondary path} (P16) with respect to \nfr{availability} and stability and 
%===============================================================================


%Given the amount of data processed and stored in the cloud by Alpha, they are also carefully considering and iterating over how they handle their secret keys, e.g. \q{definitely iterations over things [like] secret management. [...]} (P3).

%\q{A: just the scope of The scope of what can be provisioned as well as From my perspective the keys people need to have And how easy or hard it is to give people keys for that. I just find a lot of the stuff that the infrastructure level is hard to provision safely that people have keys to spin up this stuff just do certain lax. Like if if with an Amazon you give ho everybody has an account or something that you can give people right within their account, but we don't have that. So it's a lot harder for us to give people access to do that provisioning. Whereas within kubernetes the namespaces work of quite nice. It's really easy to give people the ability to just do that.} (P3)

% \q{So yeah, we're going to have more \nfr{security} stuff into our pipeline. We've only just recently kinda started researching at least I have there's a whole ton of projects like at DevOps days. I was talking to some of the government guys about their change \nfr{security} pipeline stuff and all the tools they used for scanning and there's there's a lot of out there  and yeah so package scanning would be big for us some sort of like sort of stuff that would sit on our Network and scan stuff in a would that be continuous for what would be going on to so some networking scanning stuff that looks for known vulnerabilities in our stack this kind of poke around on its own schedule for What's going on would be a really lovely thing to have here} (P12)

% end with this
%As previously mentioned an NFR may be achieved through a third party tool without the organization even realizing of the full implications of such a tool, e.g. \q{It's good to at least understand there are actual non-functional requirements, these NFRs are part of a system is a lot of time you just go through the motions and do things and not realize oh wait, these are actually processes and requirements and such.} (P3).
%===============================================================================

%===============================================================================
\subsubsection{Write Your Own Tool to Check the NFR}
%===============================================================================
As opposed to offloading NFR achievement to a third party or tool, organizations also wrote custom, in-house source code, custom tooling, scripts, or manifests \hist{ImplOfNFR}{78}{}.
For example, organization Alpha, in order to achieve \nfr{configuration management} NFRs, implemented Terraform\footnote{Terraform is an automated cloud deployment scripting language} scripts, which then largely handled deployment and operations concerns.
%, you document some infrastructure design decisions as code, which are then an integral part of the continuous pipeline and the importance of getting them right the first time, \q{a lot of those design considerations and non-functional requirements that go on, am I going to talk about how was the response time for example that dictates initial architecture and that has a huge impact. So you end up, if you're lucky you end up with a trivial use case. It's like, oh that's what that's designed for. And that's what that's designed for. You only do it once. You have to really worry about the \nfr{scalability} because it works out}. This is important to company Alpha because their business model relies on them being able to handle a large amount of data

Beta codified some \nfr{usability} parameters of their user facing front end. This codification is done as part of their source code. They submit the source code, wait for the source to process through the continuous pipeline, and finally observe and verify the result, \q{this is how we define \nfr{usability} and make sure that it's there. If you want to change our \nfr{usability} parameters or whatever we change it in source code and then we can test it and verify that it still meets our needs} (P10).

%Custom tooling (~\histogram{histogram/customTooling.tex}~) was discussed by only eight interviewees, thus much less prevalent than third party tools.
Custom tools are usually considered as a last resort where the existing off-the-shelf solutions either do not exist or do not sufficiently meet the user's particular requirements.
A custom tool may be based on an augmented third party tool that requires significant modification to meet the specified needs, e.g. \q{So we used to have <redacted> dashboards out there. But I think that we were feeling that we weren't getting enough customization out of it because it was just the metric <redacted> was giving us directly of the instances and didn't give us any application specific information} (P14).

Some custom tools were used to handle NFRs from an operations perspective to determine \nfr{availability} \histno{AvailabilityNFR}{39}{} or \nfr{stability/reliability} \histno{StabilityReliabilityNFR}{41}{} of the infrastructure, e.g. \q{I think we have a script running that gets health checks of our servers, and I think it's automatically knowing if something goes down---if they're not getting that health check then they're posting to our channel and then the appropriate person will get notified and they'll put those servers back up} (P11).

Other custom tools were developed to help automatically enforce or validate \nfr{security} \histno{SecurityNFR}{68}{} within a continuous pipeline: \q{So there's a lambda that runs when you make a bucket, it triggers and goes 'you didn't encrypt', it turns on encryption, tells you, 'you are an idiot'. \nfr{security} non-functional requirement!} (P4).
%
%Finally, custom tools were implemented to help manage data integrity and \nfr{reproducibility} when updating or creating databases as part of a system as part of an automated pipeline when implementing changes in an production environment, e.g. {I actually just redid how that flow work that used to be manual and there were a couple of instances now we're you know on I'm staging you're experimenting so your bit slower. So you type it in and it works. And all the good and production comes and you want to get it out quickly. So you go and then I wound to making some mistakes up manually updating, so now I've created a bash script. Basically the script read that file kind of does a diff figure out what needs to change and update the new database table.} (P18)
%%===============================================================================
grbage 

%===============================================================================
\subsubsection{Put the NFR in Source Control}
\label{sec:res_transfer}
In a continuous context, communicating NFRs to one's team is vital.
In the organizations we studied, the workforce was constantly changing (typically growing), and the products undergo a rapid pace of change.
The constant change requires that developers gain a clear understanding of the NFRs of the product so they know how their changes might impact these NFRs. 
Typically communicating NFRs does not include natural language documents: \q{with respect to codifying something vs documenting it: it's not precise enough it's written in English. It's open to interpretation.} (P17)
Instead, our results show developers captured NFRs directly in source control. 
`Codification' refers to using code and related artifacts (such as version-controlled JSON config files) to capture NFR knowledge \hist{Codification}{92}{}. 
For example, automated dashboards monitor health indicators such as \nfr{availability}. The dashboard contains explicit rules or triggers measuring the state of the NFR.
%Terraform\footnote{\url{terraform.com}} scripts capture NFRs related to deployment infrastructure, such as memory allocation.
Codification helps set an objective metric for developers who might not have had enough time to acquire the tacit knowledge about what constitutes an acceptable NFR threshold.
P17 notes the following: 
\q{My understanding is that we should be able to see our tests in source control in terms of nicely capturing results in a way that I and the other developers can see and say some data is not captured yet} (P17)
Other NFRs are captured in source code directly: \q{So it's in code in source. This is how we want all our pages to look this is how we want everything to function [...] That's documenting it essentially} (P10).


==> 05b_results_challenges.tex <==
%===============================================================================
\subsection{Challenges}
%===============================================================================
While the organizations in our study have concrete strategies for managing NFRs, they still face challenges when operationalizing NFRs \histno{Challenges}{71}{}.
%. 15 out of 18 of our interviewees experienced challenges when operationalizing NFRs 
The most often described challenges were difficulty using tools and tests with NFRs, difficulty prioritizing NFRs, and challenges with implicit knowledge transfer.

\subsubsection{Not All NFRs are Easy to Automate}
Some NFRs, such as \nfr{usability}, are intrinsically difficult to test through automated means, e.g. \q{I have done some [testing] using [UI test tool] selenium. Selenium is not fun. There's only one way you can test those things, for a human [to] sit down} (P4). 
%: \q{I find testing UIs is a very difficult process} (P4). 
% In the sample quote, the interviewee voiced his concern towards testing \nfr{usability} NFRs and subsequently voiced their frustration towards automated UI testing tools: 

Another automation challenge is related to adopting continuous approaches to development, which means committing and deploying at a much more rapid rate than before. For an organization like Beta that relies on manual \nfr{usability} acceptance testing for any customer-facing software deployment, the people tasked with testing \nfr{usability} become a bottleneck in the continuous process:
%\todo{this is a great quote, but it is pretty obvious who said it. } 
\q{[User acceptance testing is] easier to chunk into one deployment rather than 12 a day.} (P7).
%[The deployments becomes] a bottleneck I think [at] times for us. From my perspective once maybe twice a day is probably a reasonable number [...Anything more] I feel like would be a little bit of a challenge on the operational side to keep up with that}} (P7).
% \nfr{usability} is hard to test, as it is in other settings, but \nfr{usability} is especially difficult in SMEs where often only one person is in charge to test \nfr{usability} if automated tests are unreasonable. 

In addition to \nfr{usability}, it may be difficult to write automated test for other NFRs: 
%\q{We've tried a couple times but we haven't been very successful with the [tests]} (P16) and 
\q{There's a lot of variability and it's hard to write really good thresholds of what is working. What is not working} (P14).
Although some NFRs may not require much work to automate, based on the interviewees' sentiment, producing the ``right'' automated tests may require more than one test creation iteration. 

Furthermore, purely increasing the number of tests does not equate to higher quality tests: \q{I think that testing itself [is a] quality metric. So we're looking at coverage as a possible metric but we're trying to determine a more accurate form because we don't believe that [increasing] code coverage [will] provide us the value [...] if you test all cases that you have 100\% coverage, it's not really scalable} (P16). 

Under normal circumstances, it can be difficult to predict a sudden spike in user activity.
If Gamma suddenly experiences overwhelming levels of traffic, prior tests for \nfr{performance} and \nfr{scalability} may not suffice: \q{I feel like [tests] always [had] a bias toward the happy cases [...] When something does go wrong, it's something horribly out of left field [...] How do you prepare for those? How do you think about what left field is?} (P18).
Determining the parameters and conditions that would effectively test the entire problem space of an NFR is difficult.

% A key concept of continuous practices is the rapid collection of feedback from customers to improve a software. 
% However, when an organization fails to effectively test its NFRs or developers received minimal feedback from tests, the feedback loop facilitated by continuous practices cannot help treat NFRs: 
% %\q{But as a developer, I don't see much of that [\nfr{usability} and learnability] feedback unless it's gone through product. So 
% \q{[...] the only understanding of the \nfr{usability} of the page for me is how I [and other developers] use it} (P11).
% Without receiving testing and usage feedback, the interviewee cannot exert efforts to improve \nfr{usability} as desired by customers.
% Testing NFRs represents an important aspect of an organization's adherence to a continuous practice and good RE practices. 
% Yet, based on our study, automating the testing of NFRs is not without challenges. 


%===============================================================================
\subsubsection{Functional Requirements Get Prioritized Over NFRs}
%===============================================================================
% Make the main point of this section that NFRs are easy to drop when resources are tight. 
% NFRs become a FR when NFRs become a problem.
Since our collaborating organizations are still small and growing rapidly, employees balance many other responsibilities, among other potential limits to resources. 

In resource-constrained environments, NFRs are an easy target to bump from the sprint plan or milestone due to lack of clarity around how to test or define an NFR.
In Alpha, one aspect of their system is the need for CPU power to process large volumes of data. 
However, if not enough developers are available to maintain the system, \nfr{efficiency} and \nfr{performance} may degrade over time:
\q{Nobody's looked at this last six months maybe someone should check it out [...] It's a resource management issue and a lot of times you have too many things for too few people. [People] kind of make things and then go on to the next thing} (P4). 
An organization may be obliged to make trade-offs with the hope that immediate, short-term success will lead to the ability to remedy the trade-offs, i.e., potential technical debt, in the future. 
In our study, 14 out of 18 interviewees \histno{TradeOff}{41}{} acknowledged the existence or previous existence of trade-offs: \q{The sort of startup code today some of it you could consider clever but you do too many clever things then rack up a lot of technical debt} (P5). %and \q{It's mostly just down to just I call the law of raspberry jam. I phrase it as you can only spread things so thin before [it] doesn't cover everything} (P3). 
%In this instance, the interviewees implied that a startup organization may willingly make trade-offs for present success. For example, choosing \nfr{deployability} over \nfr{maintainability}, \nfr{performance} over stability, or \nfr{usability} over \nfr{readability}.

An organization, even an early-stage small organization, needs to be aware of these NFR trade-offs so that it can ensure that an important NFR such as \nfr{scalability} is improved when the NFR reaches a low point: \q{Some of the core pieces of the system again get more love or more time to knock that [technical debt] number down or we just pay more close attention [...] That's what always a constant battle between resources.} (P5). 
% an organization must be strategic when choosing prioritizing the issues to fix: 
% knowingly write code that may cause technical debt and problems in the long term, but in the interest of quickly delivering value to customers, an organization may temporarily accept the trade-off.
%Moreover, when an organization does intend to address its technical debt, limited resource may restrict the organization's resolve. 

% Fortunately, our interviewees for the most part recognized that limited resources is a challenge to operationalizing NFRs. Once an organization is able to direct more resources, this recognition may be act as a catalyst to alleviate these challenges. 
%===============================================================================

%===============================================================================
\subsubsection{Lack of Shared Understanding of an NFR}
A shared understanding of an NFR implies that everyone involved with the NFR is in agreement with what that NFR entails. This shared understanding relies on knowledge transfer from the people---such as the product manager or CEO---who created the NFR, to those whose work might affect it. 
Shared understanding is a challenge for our subject organizations.
They faced problems with inconsistency in what gets explicitly stored in source control; with tacit knowledge and a low (bad) bus factor \cite{Cosentino2015}; and problems with role siloing. 

Our study found organizations relied inconsistently on documentation for knowledge transfer of NFRs \histno{KnowledgeTransfer}{78}{}.
Normally, when an objective measure of an NFR exists, it would be part of the monitoring infrastructure. 
For example, the requirement that page load time is less than 500 ms is an objective measure.
When an objective measure does not exist it becomes a matter of developers' subjective interpretation, which leads to different interpretations as to what success criteria are for that NFR. 
Explicit NFR knowledge transfer \histno{knowledgetransferANDexplicit}{55}{} occurs when a developer relies on a formal metric or artifact, such as documentation, to frame their understanding of whether an NFR is being met.
For instance, in reference to having their infrastructure run by Terraform to deploy using Kubernetes, one of our respondents mentioned: \q{Aside from it being the new hotness? (laughs) It allows scaling in different ways. At least that's a big incentive for me is the idea that I don't become a linchpin and at the same time a bottleneck being the one person specialized in this or having a small team of people who are specialized in it, but that it centralized that knowledge which to me is important for scaling up things quickly} (P3).
Our subject organizations do not consistently invest effort or resources in documenting NFRs.
While some NFRs are being actively monitored (see section \ref{sec:res_metrics}) or are documented as code within a source control system (see section \ref{sec:res_transfer}), others are not.
For example, in reference to the fact that the \nfr{performance} of a feature requires processing to finish within 2.5 hours: \q{No, I don't think I have that specifically labeled. I don't think I outlined any specific requirement like that} (P2).

% Bus factor
Another problem is that knowledge is often implicit, relying on one or two people who have the overarching view (typically early employees or founders).
\q{I know a lot of the team leads have a ton of non-functional requirements in their head and how things should work and they're kind of the ones gating what goes out based on those undocumented non-functional requirements. If we were to document those we could get those ideas into the heads of the people actually writing the code, and better the development experience} (P13). 
Without transferring the knowledge of NFRs to front line developers, awareness of the importance of particular NFRs is lost. 

Implicit knowledge transfer of NFRs \histno{knowledgetransferANDimplicit}{29}{} occurs when someone on the development team attains a personal understanding of an NFR without relying on an established metric or artifact.
For example: \q{At the moment it is tacit knowledge and unfortunately when a new developer comes in and starts working on stuff [they struggle]} (P10). The `bus factor' \cite{Cosentino2015} captures a major problem with implicit knowledge: \q{I try not to get hit by a bus. So does <redacted>. Certain parts of the system are maintainable because certain people know how they work versus it being [explicitly] documented} (P5).

% boundary object/silo of roles
While explicit knowledge is captured in source control (see \S \ref{sec:res_transfer}), role siloing makes understanding the artifacts difficult \histno{SiloOfRoles}{51}
For example, capturing NFRs in the deployment scripting language Terraform is likely highly useful for team members working closely with deployment and DevOps roles, e.g. \q{For anything that I do, it [infrastructure as code] ends up in Terraform as a form of documentation} (P3). 

However, the value of documentation provided solely by code can vary depending on developer context. Developers less familiar with Terraform may have different interpretations of what the script is measuring, if they can understand the Terraform language in the first place.
The lack of familiarity makes awareness of the importance of a particular NFR more challenging: \q{maintaining the servers is like more of a DevOps role [...] whether the server is up or down is something that does get reported on to our slack software, and the whole company will see if Node goes down or something [...] it's not really my wheelhouse} (P11).

Shared understanding of NFRs relies on making knowledge explicit but also understandable, which may explain why merely capturing NFRs in code is insufficient.
%P9 believes that the feedback loop from the continuous pipeline has forced development to include documentation as part of their definition of ``done'': \q{So that sort of feedback loop for them has really helped make documentation a formal part of our [...] done ship process} (P9).

% \nfr{usability} testing is hard, as it is in other settings, but the startup means often only one person is in charge
% for other NFRs, writing good automated tests is hard, as it is other places, and in their rapid context, these tests are constantly rewritten
% quick feedback is hard in startup for NFR

% \q{There's a lot of variability and it's hard to write really good thresholds of what is working. What is not working.} (P14)

% \q{the trade-off for writing documentation and procedures is actually, starting to show up, where that would be more valuable to the company in terms of money} (P4).
% \q{sufficient testing and documentation and understanding [...] lower [the] barrier to on-boarding when [new employees] come in} P18.

%


% Lack of objective measures for NFRs in agile organizations was also noted in literature by Sch{\"o}n et al. \cite{schon2017agile} and Alsaqaf \cite{Alsaqaf2019}.

% The second problem manifests itself as a practice which organization Alpha has adopted in order to train newer team members to acquire that tacit knowledge of NFRs, their scratch environment.
% The scratch environment is described as:
% \q{We do have an entire kubernetes cluster that is just kind of a scratch base. So people have more access within that then they do in the production type environments} (P3). 
% The scratch environment serves as a place where developers can experiment with code that might impact NFRs, without affecting the production system.

==> 06_old_5.1.tex <==
%===============================================================================
\subsection{Continuous Software Engineering Supports Achieving NFRs}
%OR, "CSE supports verification of NFRs"
%include 5.2, 5.6, and 5.7
%===============================================================================

%===============================================================================
From previous literature we know that NFRs are notoriously difficult to validate or verify \cite{Nuseibeh2000, borg2003, Eckhardt:2016}.
%Although some research does indicate that NFRs can be verified by leveraging continuous practices \cite{paixao_interplay_2017}.
Even when NFRs are verified, the tests are largely manual \cite{leppanen_highways_2015}, not allocated an appropriate amount of verification time \cite{Petersen2010TheEO}, or simply left until the last minute \cite{nilsson_visualizing_2014}.
Not only do organizations not provide appropriate attention to NFRs, NFRs are cross-cutting in nature and may be difficult to decompose into fragments that can be completed in a short rapid continuous iteration \cite{bellomo_evolutionary_2014}, which further complicates the ability of an organization to automate an NFR.
Due to the cross-cutting nature of NFRs, NFRs are even more difficult to manage in larger organizations \cite{Alsaqaf2019}. 

Our evidence shows that a shift to continuous software engineering \cite{Fitzgerald2014}, makes NFRs easier for an organization to verify. 
The three organizations we studied were successful in verifying a variety of NFRs by leveraging continuous software engineering practices. 
Continuous software engineering practices can support NFRs through three key steps: 1) metrics, 2) feedback loop, and 3) continuous monitoring; all of which are necessary.
%By first identifying key metrics, an organization may create effective tests for NFRs. 
%The pertinency of an NFR largely depends on the specific domain an organization is operating in.
For example, Gamma tracks \nfr{usability} metrics through their continuous software engineering practice, including user events such as button clicks, page views, and navigation traces. 
Based on similar usability metrics, Beta runs large scale experiments and A/B tests \cite{Gupta2018}. 
These tests are used to statistically quantify and monitor the \nfr{usability} of one approach to another.
By leveraging metrics, the feedback loop, and continuous monitoring, Beta and Gamma have near-constant understanding of the achievement of \nfr{usability}---an otherwise difficult to verify NFR \cite{yu2020utilising}.
Next we will describe how metrics, feedback loop, and continuous monitoring are mutually beneficial. 
We will use \nfr{maintainability} to exemplify the three steps of achieving an NFR.

%===============================================================================
\subsubsection{Metrics}
%===============================================================================
%The primary method of verification was using NFR metrics.
%Through the use of metrics our partner organizations were able to achieve acceptable amounts of continuous verification, compliance, \nfr{security}, \nfr{usability}, run-time monitoring, and innovation as described by Fitzgerald and Stol \cite{Fitzgerald2014}. 
Assigning metrics to NFRs is not a new idea and has always been a recommended practice to ensure proper verification of NFRs \cite{bass_software_2012}. 
Metrics, of any kind, are the starting point that allow an organization to set goals, track progress, and monitor the state of the system in a reliable fashion \cite{neely_continuous_2013}. 
Given that many NFRs represent architecturally significant system requirements, the ability to create metrics and monitor NFRs becomes invaluable to an organization.

%When an objective metric of an NFR exists, it can easily be part of the continuous monitoring infrastructure. 
%For example, the requirement that page load time is less than 500ms is an objective metric.
% two examples of objective metrics -- which are easy
For example, \nfr{maintainability} has commonly been verified through static code analyzers \cite{janus20123c} that provide a number of metrics.
One such metric is code complexity \cite{mccabe1976complexity}---a lower code complexity indicates more \nfr{maintainable} code.
%\todo{@DANA: added example with acceptance criteria}
With an objective metric, such as code complexity, an organization is able to set acceptance criteria that must be met (e.g. fail the build if code complexity \textgreater 50). 
%For example, a simple block of code with no control statements would have a code complexity of 1; whereas a code block with a one single-condition \texttt{if} statement has a code complexity of 2.

Metrics and acceptance criteria can be objectively created for many NFRs (e.g. page load time shall be less than 500ms), which can be tracked through an organization's continuous monitoring infrastructure.
Each organization needs to determine which NFRs are important and create metrics---some NFRs may be more difficult than others.
As previously noted both Beta and Gamma were able to create objective metrics for \nfr{usability}.
%When an objective metric does not exist it becomes a matter of developers' subjective interpretation, which leads to different interpretations as to what success criteria are for that NFR.

However, even if an objective NFR metric is achieved, the acceptance criteria itself may be subjective or more complex than a simple pass or fail.
Thus, simply hard coding the acceptance criteria for a metric may difficult.
Rehman's \cite{rehmann2016performance} work provides a domain-specific example on how to dynamically adjust and manage the acceptance criteria for a database \nfr{performance} metric; however, the technique must be broadened and generalized.
%The concept of ``ratcheting'' a metric may also be applied to NFRs \cite{ratcheting}.
%Even without continuous software engineering static code analyzers have been used in isolation, either on developer's local machine or by a team responsible for running and analyzing the results of static code analysis (Step 1: Metrics).
However, metrics on their own are only so useful; more important is how an organization responds to a metric, through subsequent steps such as the feedback loop and continuous monitoring.

%Rehmann et al. \cite{rehmann2016performance} found that \nfr{performance} improvements or degradations must be defined in such a manner where the thresholds can be dynamically relaxed or strengthened depending on predefined thresholds, a prime example of a novel approach in applying metrics in continuous infrastructure.

%===============================================================================
\subsubsection{Feedback Loop}
%===============================================================================
In addition, metrics are even more useful if a developer receives automated feedback with respect to how a particular commit affected a metric, either negatively, positively, or entirely neutral. 
One affordance of continuous practices is the removal of manual steps in favour of automated steps, in particular manual verification, which is ``slow, error prone, and not methodological'' \cite{neely_continuous_2013}.
Much like functional tests, NFR tests should complete as quickly as possible to fully leverage the feedback loop.
Further, although a feedback loop may provide meaningful metrics regardless of the response time of the feedback, a \emph{quick} feedback loop ensures that feedback is up-to-date with fast moving requirements that coincide with the rapid development cycles used by a continuous organization. 
Exactly \emph{how} quick a feedback loop must be to be effective is yet undetermined and we believe is an area that merits future research.
Through continuous software engineering an organization is able to fully automate NFR verification through the use of two mutually beneficial practices---metrics and a quick feedback loop. 
For example, continuous software engineering supports \nfr{maintainability} by providing rapid and transparent feedback when the results of a static code analyzer are automatically compared to the acceptance criteria in a central location, i.e. the organization's continuous software engineering pipeline, that anyone in the organization should be able to access. % (Step 2: Feedback Loop).

In our study all three organizations struggled to tighten the feedback loop to make it as quick as possible.
The biggest challenge is to decrease the build and test case execution time.
The most obvious way to tighten the feedback loop is to reduce the build and test case execution time, which can be done by parallelizing builds and test and adding more computing power; however, this may be difficult or expensive.
Other strategies to tighten the feedback loop include executing a subset of tests on every cycle and running the full set of test suites less frequently.
Alternatively the feedback loop can be tightened by altering the development workflow and changing in which development activity test cases are executed (e.g. pull requests \cite{rayana2016gitwaterflow}).

The quick feedback loop may alleviate two challenges when assessing cross-cutting NFRs with metrics.
First, small changes in an NFR metric over time are hard to trace back, as there is no single event to cause a change.
Second, when multiple commits occur in a short period of time the effect on an NFR metric may be difficult to distinguish.
While these two challenges represent areas for future research into the traceability of NFRs, their consequences may be lessened through continuous monitoring.

%===============================================================================
\subsubsection{Continuous Monitoring}
%===============================================================================
Challenges with metrics and the quick feedback loop may be partially overcome through the use of continuous monitoring.
Continuous monitoring is the final key step to achieve an NFR in continuous software engineering and includes how an organization responds to a particular metric.
Continuous monitoring enables an organization equipped with metrics and a quick feedback loop to track, audit, record, document, and respond to various metrics over time.
%Metrics and the quick feedback loop would not be as useful without continuous monitoring, the longer it takes an organization to respond to deviation in the value of a metric the more context is lost, in particular with respect to source code.
For example, if the \nfr{maintainability} metric suddenly jumped from 20 to 25 and is continuously monitored by an organization, then the organization can quickly respond to the change in \nfr{maintainability}. %(Step 3: Continuous Monitoring).
An organization's ability to quickly respond ensures that those responsible for the code change still have the change context fresh in their mind.
%When an organization is creating an NFR metric the threshold of when that metric is acceptable might be difficult to discern; however, continuous monitoring can allow an organization to observe the NFR metric for a period of time to assess an appropriate threshold (which may be dynamic).

Furthermore, metrics and the feedback loop also offer traceability and transparency by allowing anyone in the organization to easily trace changes in a particular NFR metric, back to a localized change in the code.
Traceability in a continuous context has been previously studied in the Eiffel approach \cite{Sthl2016}; however, the Eiffel approach is aimed at improving the continuous pipeline, not necessarily the resulting software.
The authors \cite{Sthl2016} note that further work includes extending Eiffel to consider development activity, which would ideally include NFR activities as well.

% \todo{consider removing this paragraph?}
% Another affordance of continuous practices is the removal of manual steps in favour of automated steps, in particular manual verification, which is ``slow, error prone, and not methodological'' \cite{neely_continuous_2013}.
% Although a feedback loop may provide meaningful metrics regardless of the response time of the feedback, a \emph{quick} feedback loop ensures that feedback is up to date with fast moving requirements which coincides with the rapid development cycles used by small, agile organizations. 
% The inability to fully automated NFR verification may inhibit an organization's ability to take full advantage of continuous practices.
% For example, our study organizations still had a human in the loop for several NFRs. 
% When it comes to website \nfr{performance}, for example, Gamma has a developer manually check load-times: \q{I really do think it's more of a feeling for user [...] Just taking too long today.} (P18)
% This manual verification lengthens the feedback loop \cite{humble2018accelerate} in a continuous practice, which represents a trade-off as the organization cannot receive the full complement of continuous practice benefits.

% \todo{consider removing this paragraph?}
% Our study also revealed that an organization may write their own tool to create metrics for an NFR; although as a last resort for a resource constrained organization.
% Although writing your own tool may be the only option, especially for platform specific tools that are not widely used or in a niche domain, such as programmable controllers \cite{bougouffa2017scalable}.
% %Nonetheless, the implications are equally important, as the tool may result in a ground breaking tool (i.e. silver bullet) for a particular NFR that has immense benefits.
% One interesting NFR at Gamma involved a customized metric of organizational \nfr{revenue} \histno{RevenueNFR}{23}, which was quantified and extensively monitored by the entire organization, including development, marketing, and executives alike. 
% The custom tool enables Gamma to measure, evaluate, and assess the effect any change could have on overall revenue in real-time, including the ability to trace a delta in revenue back to a particular commit in source control.
% The tool has two notable challenges.
% First, small changes in revenue over time are hard to trace back, as there is no single event to cause a changes.
% Second, when multiple commits occur in a short period of time the effect on revenue is difficult to distinguish.

% \todo{consider removing this paragraph?}
% While proprietary software (including domain specific languages \cite{abreu2015codeaware}) has been proposed to help generalize and manage the automation of NFRs, such software has neither been implemented nor validated.
% We found that each organization has their own tools for specific NFRs and tend to be very specific (e.g. a lambda for \nfr{security}).
% The two most interesting cases are \nfr{usability} at Beta (Section \ref{sec:find_own_tool}) and \nfr{revenue} at Gamma in the previous paragraph.
% We find this area to have little relevant literature and requires deeper systematic investigation into proprietary tools and open source tools used in practice.

%===============================================================================
\begin{mybox}[Research Implication 1]
%===============================================================================
%Our results reveal that by adopting continuous practices an organization is better able to automate NFRs by defining, collecting, and monitoring NFR metrics, including otherwise difficult to verify NFRs such as \nfr{usability}.
%Due to the extremely low number of studies on measuring NFRs in a continuous context (most of which are purely theoretical) we need to further investigate approaches such as NFR metrics in a continuous context, which must be validated in industry or discovered through case studies.
%By adopting continuous software engineering practices there is an inherent advantage for an organization to achieve NFRs.
Our research has shown substantial advancement in the treatment of NFRs by defining, collecting, and monitoring NFR metrics through continuous software engineering's quick feedback loop, including otherwise difficult to verify NFRs such as \nfr{usability}.
Due to the extremely low number of studies on NFRs metrics in a continuous context there is a need for additional research to continue furthering the advancement of NFR treatment in a continuous software engineering context.
%===============================================================================
\end{mybox}
%===============================================================================

%There is a scarcity of research explicitly focusing on verifying NFRs with continuous practices. A recent systematic review \cite{yu2020utilising} identified there is a low ratio of industrial studies on NFRs with continuous practices compared to academic studies, thus highlighting the value of our industrial case study.

%There are many challenges associated with continuous practices, including difficulty in assessing continuous practices, even without considering NFRs \cite{vassallo2019automated}. Our discussion centralizes on how continuous practices affect NFRs, including practices and associated trade-offs and challenges. While these challenges may not necessarily be surprising, they are representative of the hurdles organizations are facing in industrial practices and represent significant gaps in research.In this section we discuss these three aspects: 1) how continuous software engineering practices help achieve NFRs, 2) associated trade-offs when achieving NFRs in continuous software engineering, and 3) the importance of \nfr{configuration management} as an NFR.
%However, there are associated trade-offs that are important to consider.
%We believe additional in-depth research can provide techniques or solutions to overcome these challenges, perhaps even by leveraging one of our identified practices \todo{this is ambiguous}.
% We as researchers need to realize that realizing an NFR through CI can be made possible by offloading an NFR or introducing metrics.

% We discuss our findings in terms of the opportunities, and associated trade-offs, that apply to a small, agile organization managing NFRs in a continuous setting.


==> discussion-old.tex <==
\section{Discussion and Future Work} \label{discussion}

1. interesting but not well counted themes

2. cross-company comparison (tutela vs redbrick vs ..)

3. cross-job role comparison (PM vs dev)

We should include implications for practice and implications for research (which can be inferred from the challenges to help enhance )


\subsection{NFRs and small vs large companies}


% Meetrics: allowed quantitfication of the verifiability of the NFR, and that combined with the ongoing monitoring with the feedback loop enahances the abilility and support to treating and verifying NFRs. Relate this back to the realted work and how hard it is to verify NFRs.

\subsection{NFRs as Non-Optional Requirements}

% Talk about how NFRs are not well-addressed across all three orgs because:
%   - Talk about delegating NFRs to tools
%   - Talk about delegating NFRs to cloud service providers
%   - Talk about the line where an NFR transforms into an FR
%   - Talk about the subjective nature of NFRs due to implicit knowledge transfer
% Talk about how future research should look into integrating the NFRs (as we observe them) into the requirements engineering process
%   - How should delegatable NFRs be included in the requirements engineering process?
%   - How should NFRs be documented to mitigate subjectivity (include dashboards as possible solution)?

\subsection{Relationship between Roles and NFRs}

% Talk about how the siloing of roles affects participants' perception of NFRs (definition / priority)
%   - Talk about the differing perceptions of NFRs across roles
%   - Talk about the differing priorities of NFRs across roles
%   - Talk about how management's priorities trickle down to color developers' priorities

\subsection{Relationship between Roles and Automated NFR Tooling}

% Talk about how automating certain NFRs (which are generally not automatable) can lead to workflow bottle-necks
Participant P16 told us about an interesting tooling solution to the challenge of portability across web browsers using polyfills. \q{a lot of new jobs for features come out people want to use them. [...] Can I use X? crap I can't use that because we target Safari version a million years ago. And so they include a library that fakes that feature which is called a polyfill. And so let's say something like an arrow function. It's [the library] like a little thing that will actually read your code and rewrite it to not use that feature essentially or at least big providing that feature in a liberal.} But while it is easy it is not a silver bullet. \q{We try to avoid polyfills just because they usually do impact a lot of the metrics that seem to be very important for generating Revenue which are page load times and A lot of those kind of loading related stuff.}

Quotes:
T: I would argue that DevOps takes what would traditionally takes what would be an NFR and makes it a functional requirement because you've defined it and you have to to even get your system off the ground. (Tony)

Discuss metrics in relation to outsourcing and evidence with respect to testing / validating NFRs wrt related work.

In order to provide for the NFRs, configuration management becomes the most important one. The table shows the priority by organizations, which displays configuration management as the top ranked NFR. 

\subsection{Tooling}
%===============================================================================
% Todo:

% - Explain which part of operationalization of scalability is handled by kuberenetes
% - discuss specifics that tools address
% - discuss specific challenges that tools
% - 
Based on our interviewees, another major challenge of operationalizing NFRs is tooling. As previously mentioned, all 18 of our interviewees heavily discussed the use of tools for the purposes of testing and supporting NFRs. 
Through this discussion on tools, our interviewees provided detailed challenges: \q{But that was only one team [that] actually understand like how do you run a Kubernetes cluster. Nobody seems to know how to do that} (P5). 
The interviewee refers to the difficulty of managing an applications's scalability and availability NFRs using Kubernetes. Kubernetes may help improve the scalability and availability of an application, but unlikely if a developer is inexperienced or not knowledgeable. 
A tool that does not work during critical times can have a devastating impact to an application's availability: in reference to selecting AWS regions \q{The underlying or unspoken thing about like do you spin up Amazon services in Virginia or do you avoid that because that's where it's their biggest region and so things sometimes go wrong there or they're testing out new things [...] there was one big [outage] over there [because stuff] was misconfigured}. 
For an organization that heavily emphasizes availability for its customers, even a short outage of a couple hours can cause significant monetary losses: \q{We lost like three hours worth of traffic on iOS, which is a pretty big chunk of money} (P14).
Hence, ensuring that tools positively support the realization of an organization's NFRs like availability, may be paramount for an organization's revenue. 

\section{Future Work}
The details of exactly which NFR was being operationalized is left as future work.

% Mention looking into how NFRs should be operationalized in a pipeline
% Talk about looking into which NFRs are automatable/delegatable, and which are not
% Talk about studying the effect of automating NFRs on product value?


%==============================================================================


% 1. degree of continuous software development (manual tests vs CI)
%     - can 't be partially continuous
%     - e.g. canary tests instead of manual QA test
%     - all or nothing deploys
%     \nfr{usability} testing in devops
% 2. opportunity vs control

% considerations

% Implications for Research

% For \nfr{security}, Read Seven Sins by Laurie Williams.


% 1. interesting but not well counted themes

% 2. cross-company comparison (tutela vs redbrick vs ..)

% 3. cross-job role comparison (PM vs dev)
%Steph:because quite often they don't know where the non-functional not where the non functional where the non-functional kind of concerns might creep up until they really get in there and they start to see what their what their final result is going to be so they know that they've and sometimes that's more or less apparent depending on the seniority of the developer
%Steph: So we tend to when we think about functional requirements it they're pretty hard and obvious and you know critical things and everything else sort of is just this I would say like this gray area of like you said trust that somebody else someone more technical than us knows what needs to be considered and you know, maybe some
%Steph: also expectation that we're going to see this thing before it goes out the door and that we'll know something feels wrong in terms of a non functional requirement.

% %===============================================================================
% \subsubsection{Confidence in CI}
% %===============================================================================
% Although our collaborating organizations are all practicing varying degrees of continuous practices, doubt and lack of full confidence exist against continuous practices. Eleven of our interviewees mentioned a lack of full confidence towards continuous practices at least once during their interviews. For example: \q{I don't think we've hit the point where were comfortable running Terraform scripts in a CI/CD pipeline, I don't think we've hit that yet. I don't know if we will ever be. I'm not even sure on that one. That's why I discussed with [person] and [person] a few times and I think we're unsure.} (P4). While the interviewee use Terraform to aid the organization's \nfr{configuration management} NFRs, choosing to not run Terraform scripts in consistent and reproducible manner in a CI/CD pipeline partially contradicts the purpose of practicing CI/CD. \todo{check if this inference is accurate} Another repercussions of low confidence in continuous practices include: %choosing rapid deployment over quality \q{A lot of bottlenecks and issues because people are just trying to work in smaller iterations quicker} (P13), 
% inaccurate estimates \q{continuous improvement is tricky from an estimating point of view, but you get to see results either things take a lot of time or they take no time} (P15). If a manager cannot effectively allocate development time, an NFR may not receive the level of treatment it needs. For example, if the \nfr{performance} aspect of an application took longer to realize than expected, the \nfr{security} aspect may get neglected or removed. \todo{Not sure if this is a wild inference} Furthermore, fear that continuous practices would not preemptively catch bugs before deployment is another barrier to confidence: in reference to \nfr{usability} \q{Sometimes I'm hesitant in terms of web code for that to happen because sometimes people make [mistakes]} (P4). The quote displays the interviewee's acquiescence towards automatic deployment due to the possibility of a customer facing application presenting \nfr{usability} issues.  
% Moreover, some interviewees became distrustful because continuous practices caused a bottleneck effect, where people are the bottleneck: \q{twelve [deployments] over the course of a day ends up being a lot of moving parts of communication there. That is a bottleneck I think times for us} (P7). As frequency of commits increased, a lack of automated acceptance testing in some cases meant that an interviewee suddenly faced the spectrum of not having time to do anything else other than perform acceptance tests. 
% In addition, developers may even skip the testing aspect of a deployment pipeline in pursuit of quick deployment. 
% Nonetheless, some of our interviewees are aware of the peril of not following process established by continuous practices: \q{If you're committing right to master, you'll get a rapid development cycle, but you're going to be spending the time gained on fighting fires} (P13). Without sufficient testing of NFRs prior to deployment, an organization may potentially induce more risk than than the time gained. For instance, \nfr{availability} or stability of an organization's software may be compromised when software is deployed without exhaustive testing: \q{For whatever reason that check got missed it's a manual check things got sent abroad [... resulted in software outage]} (P14).
% Ultimately, while there exist challenges regarding the operationalization of NFRs, our interviewees also provided evidence that they are aware of some of these challenges, which may provide guidance for resolving some of these challenges in the future.
% %===============================================================================




%===============================================================================

%===============================================================================
%\subsection{NFR Trade-Offs Small Companies Face}
%===============================================================================
%In this section we compare and contrast various trade-offs that a small organization may need to make with respect to NFRs in a continuous context. These trade-offs include the opportunity granted versus loss of control and manual testing versus continuous.
%===============================================================================

%===============================================================================
% NE this moved from Findings-Offloading
%(coudl use this quote) The fact that everything is running in the cloud and, as such, an organization may not have the same access as if they hosted their own infrastructure, so this provides an obfuscation by obscuring certain details from developers, e.g. \q{release stability, predictability, immutability because you don't have people fiddling around at the server like it's a one-way deploy.} (P6).
%===============================================================================

%===============================================================================
%\subsubsection{Opportunity Granted vs Loss of Control}
%===============================================================================
%As shown in our findings section, \nfr{configuration management} provides organizations the ability to use infrastructure as code (IaC) to quickly and reliably provision infrastructure. 
%When an organization is using a cloud provider, an organization can expect to create an infrastructure with ease including built-in support of important NFRs, such as \nfr{performance} and \nfr{scalability}.
%This opportunity of offloading NFRs to cloud providers might be crucial to the success of a small organization, as offloading an NFR can relieve the company of the complexity and responsibility of said NFR and allow the organization the opportunity to focus solely on the product.
%However, this opportunity comes at a cost; as an organization is now at the mercy of the cloud provider.
%In particular, if for some reason the cloud provider experiences an issue, such as an outage, an organization using said cloud provider will also experience an outage and hence the \nfr{availability} of the organization's product is now entirely out of their control.
%The removal of NFR responsibility on the part of an organization may be prudent, especially in the short term because the organization can focus efforts on delivering features of a product. 

%Furthermore, third party services can provide a myriad of benefits with respect to \nfr{security} objectives. 
%P12 describes the positive aspects of using a third party service to handle \nfr{security} at Beta in a reproducible and transparent manner, e.g. \q{I was talking to <redacted> about their change security pipeline stuff and all the tools they used for scanning and there's a lot out there [...]} (P12).
%\q{[Jenkins can] run automated security checks across that container that allow us to catch common vulnerabilities and packages and even in the application itself [...] That should improve our \nfr{security}} (P13). 
%The number of tools and services that provide \nfr{security} NFRs is indeed numerous, as P12 highlights: 
% as a developer may need to configure and setup the automated \nfr{security} checks using Jenkins.
% {[we are] continuing to discuss \nfr{security} with respect to <redacted> but I don't touch that too often, that side of things} (P6)
%However, relying on a third party tool or service to manage an NFR, such as security, may add an additional layer of abstraction, which may reduce the familiarity and understanding of how the third party treats an NFR, e.g. \q{Jenkins unfortunately for me is the magic box that I use} (P3).
%If Jenkins or the cloud provider itself has a security vulnerability, then the security issue will likely propagate to any organization that uses the service, and there is very little the organization can do to rectify the issue, except wait.

%Consequently, while a small organization that offloads an NFR to a third party is afforded great opportunity to success, it comes at the cost of losing \emph{control} over any offloaded NFR.
%In the case that an organization has a security loophole due to AWS, what ever measures the organization implements will likely have little effect on preventing exploitation of the loophole.
%Hence, the \nfr{security} NFR will only be treated \emph{when} AWS finally resolves the issue. 
%Similarly, if an organization offloaded \nfr{availability} to AWS, then AWS will ensure that the organization's product is available to the organization's customers.

%===============================================================================

%In particular, many NFRs can only be expressed in a qualitative manner; for example, usability may be described as ``The user interface must be user friendly'' \todo{find citation reference}.
%Some organizations may be hesitant to forego manual testing altogether, which may be due to lack of confidence in the continuous pipeline or automated testing. \todo{look at adoption challenges and other related work}
%Furthermore, an organization must acknowledge that the benefits of continuous will not be immediately realized; as the transition to continuous is gradual.
%According to Humble el al. \cite{humble2018accelerate}, statistically speaking, low and medium performers achieve similar percentages of manual work (with respect to \nfr{configuration management} and testing); whereas medium performers do more manual work (with respect to deployments and change approval process) than low performers; whereas high performers consistently do statistically significant less manual work (across the board) than both low and medium performers. 
%Thus, it stands to reason that an organization that is not yet truly continuous may not see \emph{any} benefit, regardless of the amount of effort exhibited.
%Ultimately, as the transition to continuous may be a difficult one, an organization must decide to either a.) forego the transition entirely or b.) commit to the transition until completion; anything in between is futile.
%===============================================================================

%\todo{consider the trade-off of keeping NFRs in certain peoples heads (to constrain other developers development so that they are in a safe space VS disseminating the information to everyone to enable everyone to be a prolific software developer!}


==> histogram/AvailabilityNFR.tex <==
1	0.833333333
2	3.333333333
3	1.666666667
4	1.666666667
5	10
6	0
7	0
8	0
9	0.833333333
10	0
11	0.833333333
12	3.333333333
13	4.166666667
14	0
15	0
16	5.833333333
17	0
18	0

==> histogram/Challenges.tex <==
1	0
2	0
3	3.5
4	10
5	2.5
6	1.5
7	1.5
8	0.5
9	1
10	1.5
11	2
12	2
13	2.5
14	0
15	1
16	1
17	4
18	1


==> histogram/Codification.tex <==
1	0
2	0.416666667
3	4.583333333
4	10
5	9.583333333
6	4.166666667
7	0
8	0
9	0
10	0.416666667
11	0
12	0
13	0.833333333
14	1.25
15	0
16	4.583333333
17	0.833333333
18	1.666666667 

==> histogram/ConfigurationManagementNFR.tex <==
1	0.333333333
2	0.666666667
3	7.333333333
4	10
5	7.666666667
6	0.666666667
7	0
8	0.333333333
9	0
10	0
11	0.333333333
12	1
13	0.333333333
14	0
15	0
16	3
17	1
18	1.666666667

==> histogram/CustomTooling.tex <==
1	0
2	0
3	0
4	1.538461538
5	2.307692308
6	0
7	0
8	0.769230769
9	0
10	0
11	0.769230769
12	0.769230769
13	0
14	0.769230769
15	0
16	2.307692308
17	0
18	10

==> histogram/FeedbackLoop.tex <==
1	3.636363636
2	0
3	5.454545455
4	2.727272727
5	0
6	3.636363636
7	0.909090909
8	0
9	4.545454545
10	0
11	1.818181818
12	2.727272727
13	10
14	0
15	2.727272727
16	3.636363636
17	0
18	0

==> histogram/ImplOfNFR.tex <==
1	0
2	0.37037037
3	4.074074074
4	10
5	6.296296296
6	2.222222222
7	0
8	0
9	0
10	0.37037037
11	0
12	0
13	0
14	0
15	0
16	0
17	0.37037037
18	5.555555556

==> histogram/KnowledgeTransfer.tex <==
1	1.111111111
2	1.111111111
3	3.888888889
4	4.444444444
5	10
6	1.666666667
7	3.333333333
8	0.555555556
9	2.222222222
10	1.666666667
11	1.666666667
12	0
13	3.888888889
14	0
15	0.555555556
16	0.555555556
17	5
18	2.777777778

==> histogram/MaintainabilityNFR.tex <==
1	4
2	1
3	1
4	4
5	10
6	4
7	0
8	0
9	4
10	0
11	0
12	3
13	0
14	0
15	0
16	3
17	1
18	1

==> histogram/Metrics.tex <==
1	0.714285714
2	0.357142857
3	4.285714286
4	5.357142857
5	3.571428571
6	0.714285714
7	0.714285714
8	0.714285714
9	2.142857143
10	0.714285714
11	2.5
12	0.714285714
13	4.285714286
14	4.642857143
15	3.214285714
16	10
17	4.285714286
18	6.071428571

==> histogram/NFROffloading.tex <==
1	2.571428571
2	3.428571429
3	6.285714286
4	10
5	9.428571429
6	1.428571429
7	0
8	0
9	0.285714286
10	0
11	0.857142857
12	2.857142857
13	2.857142857
14	0.285714286
15	0
16	3.428571429
17	0
18	0.571428571

==> histogram/NFRPerception.tex <==
1	1.860465116
2	0.465116279
3	3.953488372
4	10
5	4.651162791
6	1.395348837
7	1.627906977
8	2.325581395
9	1.627906977
10	1.162790698
11	1.627906977
12	1.395348837
13	1.627906977
14	0.465116279
15	1.627906977
16	8.604651163
17	0.930232558
18	5.581395349

==> histogram/PerformanceNFR.tex <==
1	2
2	2.666666667
3	2
4	4.666666667
5	5.333333333
6	2
7	2.666666667
8	0
9	2
10	3.333333333
11	1.333333333
12	2
13	4
14	5.333333333
15	2
16	10
17	3.333333333
18	4

==> histogram/ReadabilityNFR.tex <==
1	3.333333333
2	0
3	0
4	7.777777778
5	10
6	4.444444444
7	0
8	0
9	0
10	1.111111111
11	0
12	1.111111111
13	0
14	4.444444444
15	0
16	2.222222222
17	0
18	0

==> histogram/ReproducibilityNFR.tex <==
1	0
2	0.909090909
3	7.272727273
4	7.272727273
5	7.272727273
6	2.727272727
7	0
8	0
9	0
10	0.909090909
11	0.909090909
12	0.909090909
13	4.545454545
14	2.727272727
15	0
16	10
17	0
18	1.818181818

==> histogram/RevenueNFR.tex <==
1	0
2	0
3	0
4	0
5	0
6	0
7	0
8	0
9	0
10	0
11	1.111111111
12	1.111111111
13	0
14	4.444444444
15	10
16	2.222222222
17	5.555555556
18	1.111111111

==> histogram/ScalabilityNFR.tex <==
1	0
2	0
3	9.090909091
4	8.181818182
5	10
6	0
7	0.909090909
8	0
9	1.818181818
10	0
11	0
12	1.818181818
13	5.454545455
14	1.818181818
15	1.818181818
16	7.272727273
17	0.909090909
18	1.818181818

==> histogram/SecurityNFR.tex <==
1	1.923076923
2	0
3	4.230769231
4	10
5	0.769230769
6	0.384615385
7	0.769230769
8	0
9	0
10	0
11	0
12	1.923076923
13	1.153846154
14	1.153846154
15	0
16	1.538461538
17	0
18	2.307692308

==> histogram/SiloOfRoles.tex <==
1 4.44444444444444
2 1.11111111111111
3 1.11111111111111
4 8.88888888888889
5 0
6 2.22222222222222
7 10
8 1.11111111111111
9 1.11111111111111
10 2.22222222222222
11 10
12 0
13 6.66666666666667
14 1.11111111111111
15 0
16 1.11111111111111
17 3.33333333333333
18 2.22222222222222


==> histogram/StabilityReliabilityNFR.tex <==
1	1
2	0
3	5
4	10
5	0
6	1
7	4
8	0
9	1
10	0
11	0
12	7
13	3
14	0
15	1
16	2
17	4
18	2

==> histogram/SuperNFR.tex <==
1	3.893129771
2	3.969465649
3	6.106870229
4	10
5	7.404580153
6	3.511450382
7	2.748091603
8	1.603053435
9	3.129770992
10	3.969465649
11	3.816793893
12	3.053435115
13	4.045801527
14	3.664122137
15	3.435114504
16	5.954198473
17	2.671755725
18	4.732824427

==> histogram/TestabilityNFR.tex <==
1	1
2	0
3	6
4	10
5	4
6	5
7	0
8	0
9	5
10	2
11	0
12	0
13	3
14	2
15	0
16	6
17	1
18	2

==> histogram/Testing.tex <==
1	3.461538462
2	5
3	2.692307692
4	8.076923077
5	4.230769231
6	2.307692308
7	0.384615385
8	0.384615385
9	5
10	6.538461538
11	4.615384615
12	1.153846154
13	1.923076923
14	3.461538462
15	1.538461538
16	10
17	1.153846154
18	1.923076923

==> histogram/Tooling.tex <==
1	2.777777778
2	3.148148148
3	5.555555556
4	10
5	7.962962963
6	1.666666667
7	0.185185185
8	0.185185185
9	0.37037037
10	1.111111111
11	1.851851852
12	2.037037037
13	2.407407407
14	3.148148148
15	0.555555556
16	3.333333333
17	0.185185185
18	2.037037037

==> histogram/TradeOff.tex <==
1 5
2 0
3 1.66666666666667
4 10
5 10
6 3.33333333333333
7 0
8 1.66666666666667
9 5
10 1.66666666666667
11 0
12 1.66666666666667
13 5
14 8.33333333333333
15 3.33333333333333
16 3.33333333333333
17 3.33333333333333
18 5


==> histogram/UsabilityNFR.tex <==
1	0
2	0
3	0
4	8.333333333
5	0
6	5
7	5
8	0
9	2.5
10	10
11	5
12	0
13	1.666666667
14	0
15	5
16	0
17	0
18	2.5

==> histogram/documentationANDexplicit.tex <==
1 1.0
2 1.0
3 4.0
4 0.0
5 10.0
6 0.0
7 3.0
8 1.0
9 3.0
10 4.0
11 2.0
12 1.0
13 0.0
14 8.0
15 9.0
16 0.0
17 2.0
18 4.0

==> histogram/knowledgetransferANDexplicit.tex <==
1 0.0
2 0.9090909090909091
3 4.545454545454545
4 0.9090909090909091
5 10.0
6 0.0
7 0.0
8 0.0
9 1.8181818181818181
10 0.9090909090909091
11 0.0
12 0.0
13 0.0
14 0.0
15 0.0
16 0.9090909090909091
17 2.727272727272727
18 3.6363636363636362

==> histogram/knowledgetransferANDimplicit.tex <==
1 2.2222222222222223
2 1.1111111111111112
3 3.3333333333333335
4 4.444444444444445
5 10.0
6 3.3333333333333335
7 6.666666666666667
8 1.1111111111111112
9 2.2222222222222223
10 3.3333333333333335
11 3.3333333333333335
12 0.0
13 7.777777777777779
14 0.0
15 1.1111111111111112
16 0.0
17 7.777777777777779
18 3.3333333333333335

==> old-intro.tex <==
% Standards have been developed to aid practitioners in traditional requirements management, such as IEEE-830 (``Recommended Practice for Software Requirements Specifications'').
%The definition of a non-functional requirement (NFR) has been a notoriously controversial topic among software engineer practitioners and researchers. 
%A large part of the reason for this controversy is based on the fact that NFRs may be harder to express in a traditional sense and difficult to verify, or even validate \cite{Nuseibeh2000}.
% However, it is not clear whether these standards can be effectively used in conjunction with non-tra\-di\-tional methods, such as agile or the more recent continuous integration practices \cite{sillitti2005engineering}.
% In fact, much akin to NFRs the definition of continuous integration is not consistent across industrial organizations and the definition can greatly vary \cite{STAHL201448}.
% Furthermore, continuous integration is just one example of a growing number of continuous practices, which include the likes of continuous development, continuous planning, continuous testing, continuous finance, etc. 
% These practices are also known as continuous star (*) \cite{Fitzgerald2014}.
% Despite the ambiguity of what is exactly continuous integration, the importance and value of implementing continuous integration has many perceived benefits and thus has become a mainstream practice \cite{STAHL201448}.

% Implementing a continuous practice in a software specific domain (e.g. continuous deployment) requires software to be continually and rapidly released to end-users by using some sort of an automated pipeline.
% An integral component to facilitate a software deployment pipeline is the concept of infrastructure as code (IaC), whereby the infrastructure required by the software is ``codified'' in order to facilitate seamless and reproducible deployments \cite{humble2010continuous}.
% IaC is managed by an operations team, which is tightly coupled with the development team; in fact, the coupling is extremely tight to the point that the development team and the operation team have been amalgamated and integrated into a single entity, commonly known as DevOps.
% The associated benefits achieved by IaC are numerous, and include security, auditability, testing, documentation, and traceability \cite{johann2017}; each of which may be considered an NFR.
% Conversely, one can achieve the aforementioned NFRs by codifying, or operationalization, the infrastructure as code.
% Given how NFRs can be realized from a continuous practice, such as IaC, we were interested in researching what other NFRs could be operationalized using some form of continuous practices. \q{We're I mean devops is going towards like infrastructure as code and if we could do like could bring that idea to like more more of this kind of thing, like especially data migrations because they're always data and schema migration because they're always a risky piece of any application.} (P6)

==> results-old.tex <==
%===============================================================================
\subsection{Terminology} \label{terminology}
%===============================================================================
\todo{maybe this section goes away entirely. it introduces doubts about the construct validity. the evidence for how the backlog discusses NFRs could appear in documentation discussion}

Research question 1 asked ``How do these companies manage their non-functional requirements?'' 
In order to answer this question, we first baselined our study by examining how well our respondents understood the concept of a non-functional requirement. 
In line with previous studies (see \S \ref{method}) none of the 18 interviewees were able to confidently provide a concrete definition of an NFR, nor could they immediately explain how their company dealt with them. 
The closest definition was \q{a stipulation or a requirement of how it's done [...]} (P7).
Seven of the interviewees (P3, P5, P13, P14, P15, P17, and P18) were able to provide a definition using examples. For instance, \q{Anything that sort of impacts a property of the system. So for our systems performance falls into that} (P17).
%Reliability largely falls into that. Maintainability is definitely on our minds too

The remaining ten interviewees were unable to define what the term NFR meant. %e.g. \q{I have no real clue on how to define non-functional requirement.} (P16).
Of course, an inability to match a textbook definition does not mean our respondents did not understand the concept.
%, we do believe that many of the interviewees had a solid grasp of the concept of NFRs; however, they simply may not have been able to accurately articulate it, e.g. \q{Yeah, I guess the answer is yes, but I don't know if I can really stick it into words} (P4).
After some prompting on our parts, each respondent was readily able to articulate their perception of the concept of NFRs (\textsf{NFRperception} --~\histogram{histogram/NFRPerception.tex}~), or explain how problems they had faced were in fact non-functional in nature, e.g. \q{I think there was lots of things I never considered before} (P16).

% \todo{findrealnum}
% Furthermore, X of the eighteen interviewees had trouble differentiating between a functional requirement and an NFR, as one interviewee described \q{the magical line between non-functional and functional and where I just consider things functional but technically they're non-functional. So that's what I struggle with because I might have some but I don't know where to bring them up} (P4).
% Despite the fact that only eight of the interviewees were able to immediately provide a definition of an NFR (including using examples) two (P5 and P14) of the interviewees identified the importance of NFRs to software development, without provocation, e.g. \q{So like performance, security kind of goals or like these categories of things that are important but aren't like directly listed as to what it has to do} (P14).

% Once the interviewers prompted with examples and elaboration of the term NFR, we found that each interviewee was easily able to explain how an NFR could be addressed using their organization's continuous practice.
They could also provide many examples of \emph{how} NFRs occurred at their  organization. The code we created to amalgamates mention of \emph{any} kind of non-functional requirement mentioned by respondents was \hist{superNFR}{828}.%$~, 828 mentions). 
%These findings are in line with other research into NFRs. \cite{} 
We were satisfied that all respondents understood the concept of NFR after our explanation. 
%Once the respondents were prompted and could define NFR within their context, 
We were then able to proceed to examining the strategies used and challenges faced with these NFRs.
\todo{this could elaborate with reference to the backlog data - where no mention of NFR occurs}.


\begin{comment}
- NFRs become FRs after pass some threshold (discussion?)
- gap between textbook definition and environment(??) definition (I am not sure how/where to talk about this)s
- impressions of NFRs (SuperNFR) (discussion?)
    - by role / org didn't differ much (discussion?)

Codes:
- NFRPerception 17/18
- SuperNFR 18/18
- Development 12/18
- Merging 13/18

\end{comment}

%===============================================================================
\begin{comment}
THESE ARE EXAMPLES OF OPERATIONALIZATION
P5:
for example, like scalability just by Devops you automatically get scalability in a lot of cases for say certain web services running on Docker and  kubernetes,
They [scalability and reconfigurability] can be depending on the situation but often times now you get them for free just because of the devops tooling that you have available to you now
So you give data plural or Apache bean I guess that's what it's called nowadays by adopting that your You're inherently being it's selling point is the fact that it addresses certain non functional requirements in terms of example, this case let's say scalability. So that's it's become more common. Tools Explicitly addressing and giving the ability easily. Have those non-functional requirements taken care of or at least does that make sense?
some of those non-functional requirements you say like, they used to be it used to be a lot of them are overlooked, you know, it would be an Assumption or are it would just be as good as it was gonna get but now I mean, Because everything's running in the cloud. Usually within a certain Frameworks, right? So like if you're an elastic Beanstalk You've for a business you're running a web service and a hosted environment or managed environment on AWS. You put your web application up there and it's immediately spread across however many availability zones and notes as you want just punch in the numbers or just gives you availability for example and scalability in that case. 13:02 Just out of the box just magically have it. So people sort of assumed people start to assume that that you know, your availability and scalability should be X just because they assume your On certain framework.

One common NFR operationalization is usability through the use of metrics to validate if components are accessible and which components are accessed most.

Security is operationalized by augmenting common continuous tools to verify or validate that certain conditions are met or maintained.

Maintainability and readability, are operationalized through code style checking.

Static code analysis

IaC
Testability - ability to perform A/B testing by 
availability
scalability

Containerization
\end{comment}
%===============================================================================
%===============================================================================
\begin{comment}
P5:
T: It depends on what scale we're planning to run at. usually there's a lot, pick on databases. For example, you used to be that you could take a database you go and you know as tell you in school. when you scale it up It's going to ball up because hit a memory wall or run out of cores, you know, it's a single node. It's not a cluster blah blah ba blah. or you know, it's running this version of SQL or something. It's you just know that like, it's going to hit the cliff at some point. You also might know that you have to test it. to say, Okay Well when our when is our particular Frankenstein, it's using this database going to hit that drop off my capacity.  you have to test it ahead of time. Especially if you're going to, you know, scale it past a certain size. some of the cloud-based databases, for example, like dynamodb on like the horizontally scalable database have a much more predictable usage pattern. You can just turn the knob to get more performance, of course pay money.15:24  But like it's generally fairly easy if you follow this pattern in you know, so you don't necessarily have to get out in front of it and test it at that scale. If you don't want to you can sort of choose to roll the dice.
T: For me it comes down to how mission-critical this whether we choose to do that scalability testing or not. Same with data processing. Things like that It used to be we tested more of that explicitly, but once you're comfortable with the tools or the you've used a platform at a certain scale before. then You don't necessarily need to test each Incarnation every single time, especially if you're on the lower ended of usage. that was a tough one, because you can be super super anal about setting it up and pre-testing things but Usually you've got quite a bit of rope before you run out of it these days. So that one's, that one's interesting.
\end{comment}
%===============================================================================
%===============================================================================
\begin{comment}
P5:
huge part of it is that documentation that of the infrastructure that you're running on or  the configuration?

\q{right it's all the things you assume will happen but no one writes down} P5

\q{A: reproducibility is an important part and documentation and the way just so that how things are wired together is documented somewhere in some sort of code that prevents look through because there's also a lot of magic things that just exists and there's some process of reverse engineering those and I hate that I hate that that's a skill set of developed but it’s It's necessary on by very much like having where one of the things we even do within our stuff is are taking process is so we use it for structures coach provision things but things within the environment if they are provisioned tell us where because they come from multiple git repositories and stuff. So we have the other way saying this came from this repository. So you have a hope of figuring out what is this a part of what is it connected to so you have the ability to reason about how this piece functions within the larger system. Just kind of the way to connect the dots.} (P3)
\end{comment}
%===============================================================================

%===============================================================================
% IaC as documentation -- not sure this fits with the continuous paradigm?
%Using some form of IaC involves developer a configuring part of all of the infrastructure artifacts as code, which can later be included in source control.
%IaC has led several developers to consider the codified infrastructure files as a form of documentation.
%These files are then available to all developers who are interested in reading, and modifying, e.g. \q{that's why you like these things like Terraform because it's infrastructure as code documentation is only so good because the authoritative source of documentation} (P4) and \q{it ends up in Terraform as a form of documentation as well as the idea} (P3).

%\q{You have to go back. And revisit that. Like okay, this isn't working. It's not scaling. This is scaling but the downstream stuff isn't scaling. Because the person writing it could have written it and it's probably smart enough to have written it with some, you know, additional logic to like mitigate potential like what if the list is long situations, but with the way that you do sprints and scrums and iterative design, it would be silly to potentially pre-optimized that in the first pass and so you just sort of eventually, wait for it to fail down the line depending on proactive you are with spotting that kind of thing.} (P5)
%===============================================================================

% maintainability 
% \todo{omar}
% \todo{get maintainability quotes -- and put them either here or in implementation}

% Dependency Management (Maven vs Node)
% Source code consistency helps with maintainability
% Lack of documentation factors into maintainability (Quote -> Challenges)

% Tony:
% C: That's another yeah, that's good. Okay, so that one for us isn't a huge thing. though It definitely is a thing we try to have a decent amount of Code standards, but I would Argue that We've adopted certain code or certain standards within like Java For example where you certain libraries that make it easier to keep your code cleaner to code in a certain pattern but I wouldn't say it's strictly enforced everywhere. It's there's definitely some variability and a lot of that comes down to like most things are code reviewed its to some degree but it's like who's doing the code review and depending how core critical to system is they'll get more love or more attention in terms of like. maybe we should make sure that that's like super squared away where stuff that's more near the edges through the leaves or is maybe more initially more exploratory. You're like, okay, we're going to wire it up this way. Probably not the best way but this is as good as we could do right now with what we know is we don't know enough about the requirements for example, or you're like I hope this is good enough and configurable enough, right. because I find in terms of maintainability. There's stuff like dependency management that's baked into our process pretty tightly because we're using Maven. I'm going to pick on Java. We also use node, but luckily that's fairly standardized these days in terms of most languages have a dependency management system and a build system. So it's not too bad to keep that stuff sane. in terms of that. You want to go into the code and you want to make a little change that can be more. especially near the leaf. So get edges of the code base or even some of the data processing stuff. Can be it can be harder because it'll be coded in one way and then the assumptions or the configuration it. Oh, you can change these three options and I like good enough and then you have to something, you know, you add in two or three more options and it sort of follows the pattern it's still fairly clean, but then there's this other one weird thing that you have to like propagate through several layers of code and like that's sort of ugly, but that's just the way it is right Now. the sort of startup code today some of it you could consider clever but you do too many clever things then rack up a lot of technical debt, so 55:43
% T: The whole sort of startup technical that thing does, it happens to everyone you always have to make trade-offs in terms of the maintainability. The other side of maintainability has to do with like who can maintain it. It's like some things are very clear and like You get the coop to do it as long as you have some do a code review. I should go to look at it and get it's fairly laid out, but I mean documentation for us. is Lacking severely in a lot of places which also factors into maintainability if you don't have the documentation and it's the simpler stuff for the stuff is really laid out with a consistent pattern. That's the stuff that everyone can maintain it's easier to maintain because you don't necessarily need the diagram you sort of can follow it through and anyone who's done decent on a programming or some programming can get the gist of it without a like a specific flow diagram or some sort of this goes to this goes to this. in our case process a lot of data. So there's arrows going to boxes.
% T: That I would say like us because shortcoming in terms of maintainability has to do with either technical debt, so decisions For like this is good enough for now. we've tested it so it works but it's not necessarily like the eat we'll have to do a bigger refactor. If you want to push it further that's obviously lurking in certain parts of the system more than others, but I suppose that's true for any organization and the other side is documentation. So like I try not to get hit by a bus. So does Adam. that like certain parts of the system are maintainable because certain people know how they work versus it being like School documented

% Brian:
% B: Currently. We do not have any static code analysis, but that is a good point we could ride we could be running profilers on these and determining what our If it's any kind of cyclomatic complexity is and things like that. We don't have any static analysis

% Phil
% P: Yes. Absolutely. It's probably one of my number one concern is maintainability because that's the hardest thing to do writing codes easy. Keeping Keeping code working is hard. My current project has been going through really really old code and trying to figure what the heck it does. It's non-trivial.

% Drew:
% D: Yeah maintainability like just avoiding Tech debt such things. Where do I do it or put it it's a pretty important thing. I read a colleague's essay the other day who wrote something up comparing. Shipping things in his article is kind of putting out view. Mine was a little bit rough, but I liked what he did. He took some Anthony Bourdain quotes about kitchens and food and he put like the mise en place where everything goes as place and you work in your kitchen to like clean the chip things out and you're not even you know about this but this is all new to me and so saying like your organization like when the head chef comes over and he's your workstation and it's kind of like it's dirty God throw it out. It's just no good in like your food and you're slow and your head's a mess when it's like that and he's like as a developer you want like all your things like in the nice position so you can ship swings fast and you can get a continuous. So you get all these plates going on exactly the same every time which is kind of a goal to get to so for maintainability and I think maintainable these things that enable like all the stuff to stay in the same places. Do you be able to decode fast and discreet 18:04  I like that one. So that's something that if you prefer keeping tech debt it down and keep your tools concise and clean. that was kind of fun analogy.
% D: Repeatability. So the more you kind of cycle over stuff the more you kind of get cut on the things that aren't like clean on the edges the more dirty stuff gets and the more you repeat it and go over this process you try and simplify it down so that it works better and faster each time. So it's kind of the repetition of these small pieces is what I value. It's getting things get more maintainable the more you break them. by revisiting code. You also like you clean it up like that when I was working on some random PR today, but the more eyes and people that came through on the pull request, like will this code could be tinkered this code the more people hit the mark Cycles over. It's just kind of valuable for keeping things consistent kind of shared experience of like kind of developer standards as we're all working and talking on how we try and do things using similar tooling in the same way.
% D: so lots of things can be embedded in there one thing that22:26  Guy I used to work with really wanted was like code quality things like static analysis of code and you go through and it's just like kind of gives you like different numbers and breakdowns for like you using the more of this and more of that. The one that we were using is kind of is called we'd come up with a code format. It's like this code is quality 4 code complexity algorithms.  I don't like it was kind of like a little annoying because like what are the algorithms digging for was in this project? Not that clear but it'd be like you like a 4 your great who are like this is a 1 it's kind of arbitrary which is kind of like vague and weird, but it was also kind of nice. So there's you can put that sort of thing in the pipeline, you know, I want our pipelines here to like track stuff more. So in that sort of thing, you can just like get those little at the end of the end up Jenkins around it just spits out like a little number like this in and you can take That number to do database and you can have like a running love or you can chart it out later and be like, alright, so our code complexity is going up and then people do a bunch of refactoring you watch it change with time which is kind of kind of would be fascinating to see

% tyler:
% T: Yeah, I think we do we prioritize flexibility and maintainability a lot in our code. And I mean that that might explain why it's one of the few things we do have codified

% % readability 
% A total of 9 participants across the three organizations brought up the use of source code linters or prettifiers.
% Linters test source code files against a code style guideline whereas prettifiers, on the other hand, reformat source code files to adhere to a particular code style guideline.
% Both types of tools enforce the usage of code style guidelines (passively in the case of linters, and actively in the case of prettifiers) to enhance code readability.
% These tools are typically run within a developer's integrated development environment (IDE) or editor, or as part of the project's automated pipeline as part of their continuous practice as one participant notes:
% \q{First step convention style guides, we have those and we enforce it using many tools. So you can easily run a linter before you commit. We also run it on our CI system. so we could detect if a developer has ran the style guides and or has followed all of it} (P16).

% usability
%\todo{do we need this section?}
% brendan:
% B: we can see how many users are using a specific feature for example, so product has been very interested in that actually because we're revising lot of our application and we begin the question do we bother with that page?13:08  If only two people are using it maybe we can allocate resources elsewhere. So not only is not only is the feedback benefiting developers but product in their decisions and it's kind of pushing the application in different areas that people may not have thought were important. So that's pretty cool to see that sort of stuff.
% B: Yeah, we already hit the performance, the number of pages under the Hood. Yeah, at this point in time. It's kind of just I know product uses like user experience tracking so they can actually see how the user is using the app. But I think that's pretty much the extent of it with your gross metrics and stuff.

% phil:
% (referring to selenium as part of the build process)P: currently yes, so the builds run they get deployed and then a test runs and runs against the deployed build like a like a staging environment one and then the production. I mean currently as it stands a production Build is a button click by a human. So it's not like everything gets pushed to production. I don't like that with

% P: So the ability to quickly roll back or redeploy an older image or something along those lines. So recoverability at any point in time. So whatever environment I am deploying to the ability to recover to an older one quickly so which I think, But even, Yeah, because with UI stuff sometimes something is broken and it's really hard to catch. It's a bug somewhere something you just don’t know about. So, you know another important or the alternative is that fast fast deploy. The plane can be very quick. Which is always, sometimes challenging the more test the slower your deploy is. And depending on the tools if you're using maven and in Java, sometimes there's just no such thing as fast deploy.

% nick:
% N: So we got it out in front of customers and we realized that like the legend that defined but each of the columns was was not clear or well placed so it was there and it like met the requirement but nobody found it. Right. So getting that feedback quickly was good
% This is because of the ability to quickly release something to a customer and receive feedback, perhaps as part of a feature flag.

% marc:
% M: Yeah, so we're trying to do more and more of that.So yeah, so we're starting to do it. We're at we're just starting a project to start to codify more of the app and start locking in those patterns. So usability patterns.

% % testability
% \todo{Testability of NFRs with respect to testability of particular NFRs and testability of a particular component.}
% \todo{find homes for these}
% Testability of code is paramount to the success of a true continuous software development project.
% In particular, to ensure there is sufficient confidence in a change to the source code many of the organizations run the source code through a gauntlet of tests.
% However, it is noted that testability should not be compromised at the expense of slowing down the feedback loop, as noted \q{That's the time it takes for continuous pipeline upon detection of code change to run the entire suite, get all the environments loaded, and to execute all the tests, and return the report. I've worked on projects outside of this company where your longest test suite runs in 30 seconds. And that just provides you so much feedback} (P16).
% Interestingly, one organization noted that they still perform manual testing as they have yet to automate the testing; however, this is not due to the testability of the code, it is a prioritization issue.
% Notwithstanding, the organization does understand that value in automating the tests within the pipeline to achieve the full benefit, e.g. \q{even though we don't automate the testing on that there's a manual process for doing the testing before we push something to production. It isn't testability issue. It's just a we didn't get around to automating it issue. So that is something that's on our list to especially the staging environment because we can just then we'll continual testing} (P5).

% In addition when offloading NFRs to third parties, there is a trade off of relying on the provider to meet service level agreements versus performing your own testing to validate the level of service, e.g. \q{it's generally fairly easy if you follow this pattern in you know, so you don't necessarily have to get out in front of it and test it at that scale. If you don't want to you can sort of choose to roll the dice.} (P5).

% Furthermore, IaC can aid in the testability of a software component or system.
% IaC allows a developer, tester, or any other employee who so desires to simply run some component or system through the codified scripts, e.g \q{infrastructure as code can definitely help with that depending how much you need to have in place in order to run things. Whether that's to the extent of you fire up Mini Coop, and then it's firing up a series of containers and you have full test environment or if it actually provisions you could provision whole underground infrastructure on Amazon with in some safe test environment. So it can definitely Empower people to to put in place a lot more tests pictures or environments like that. It's really easy for people to spin stuff up locally on a local test environment. They can spin up a Kubernetes cluster and test things within it} (P3).

% Similarly, availability is often manually tested: Regarding availability\q{Yes, 100\% we can definitely automate more manual tests} (P16). In this context, the interviewee admits that more automated tests would be beneficial. 

%===============================================================================
% Even when the right automated tests are created and added to an organization's deployment pipeline, maintaining automated tests is another challenge: \q{We've had some experience with bloated end-to-end suites for example, and those tests are like heavy and difficult to maintain} (P9). 
% Essentially, this interviewee discusses the long term challenges of tests that help operationalize NFRs in an organization. In other words, tests like software have important pertinent NFRs that may accumulate technical debt and reach a ``bloated'' state when neglected. 

% In addition to tests, the resource challenge may affect every aspect of an organization: \q{I already knew one we're completely under resourced to this project was way too big and it basically had one person and that's insane} (P8). 
% Although not directly explained, we can infer from the interviewee that too much responsibility may be placed one person. Instead of properly testing the software and ensuring maintainability, person may opt for deployability to swiftly release the product. % NE not controversial
%\q{they setup an experiment worker at the front gets deployed to say X percent getting this and X percent getting. my understanding of that we should be able to you know should be able to see all those things enter code in Source control passing through. in terms of nicely capturing results in a way that I and the other developers can see and say oh this is that we're not there for the capture yet. not that People aren't capturing the data for themselves but it's not it's not formalized.} \\
%As part of their testing process certain NFR checks are codified.
%This is further echoed by P3 when they mention using a sandbox as a test environment for developers to experiment with:
%\q{ It's really easy for people to spin stuff up locally on a local test environment. They can spin up a kubernetes cluster and test things within it. We also have a scratch environment that people have a lot of access within.} 

% Codification Quotes
%P5: huge part of it is that documentation that of the infrastructure that you're running on or the configuration (with respect to IaC)
%P5: well now  there's Jenkins files the Jenkins files in the repository. It's versioned it spells out exactly what the build is going to do.
%P16: So I guess to answer the documentation aspect of this it would be mostly within code.
%P3: it ends up in terraform as a form of documentation as well as the idea.
%P4: that's why you like these things like terraform because it's infrastructure as code documentation

%P6: That's a codified set of design standards that are in place for for our company to use and wrap it when we can use it to rapidly build things build interfaces that that adhere to our design our design standards.


%In person knowledge transfer, i.e. talking to someone
%P4: clue in better as to what is functional and non-functional how to plan Those things better into projects. My responsibility is planning a lot of things and I don't always. These things are in my brain. I don't always express themselves
%P1: There'd be more mentoring than just Although I expect if somebody were to join onto my project. There'd be more mentoring than just ""here you go figure it out yourself""
%

% - Explicit docs and bus factor
% - Codification... using the code to explain why/how the NFR can be met - e.g. documenting deployment approach. Some use of comments\\

% \q{T: yeah, I mean, I think I'm a little bit missing how to codify some of these non functional requirements.} (P6)

% \q{M: sure we use mostly Amazon services at least for hosting running code as well as GitHub. So most of the stuff that we do is has to be made as cloudformation template it's kind of frowned upon to directly create stuff in the console because that you're not tracking you don't know where it is to be rebuilt. Nobody knows how things just get just kind of like having magic numbers in your code. You know, like you don't want to just have stuff out there that's not listed in some form and not easily able to be reproduced. So all of our stuff is in cloud formation templates and we use the Amazon cloud formation in our deploy  pipeline to automatically adjust what stuff is provision when you push a change} (P14)

% \q{M: they. We're trying to document them. We're trying to document them, establish these patterns so they are in code. So for example right now or one of the things I currently built is like a page component which encompasses the entire page with a page header and tabs. So that's a pattern that we want to start using it throughout the app. So it's in code in source. This is how we want all our pages to look this is how we want everything to function.That's somewhat document. That's documenting it essentially.} (P10)

% \q{T: Yeah. Yeah. I'm trying to think of what could be codified. That's like other than like infrastructure. Oh, I guess code quality stuff like linters and things like that. That's all codified. Actually now that I think about it and like our formatting we use will on the front end. We use prettier for formatting and it's all in code like and then are we use eslint as well.Catching errors and and enforcing best practices. So it's all in code} (P6)

% \q{T: Yeah, I think we do we prioritize flexibility and \nfr{maintainability} a lot in our code. And I mean that that might explain why it's one of the few things we do have codified} (P6)

% \q{T: Yeah, fair. That's a codified. I mean sticking with the codified theme. I think that's a theme here. That's a codified set of design standards that are in place for for our company to use and wrap it when we can use it to rapidly build things build interfaces that that adhere to our design our design standards.} (P6)

% \q{C Are the margins in the code? That is something that we are getting into the code now. We have a mock that figures out how to best get calculate variance and keep it accurate across any aggregate of the data so that I can have that value when I create the diagrams.} (P2)

% \q{Q: it's not codified in source control. A: no. Q: do you think it can be? A: yeah, oh yeah. I keep begging at people to, I only have so much influence} (P3)

% \q{B: we can codify it. I think you could codify those metrics. We haven't done it but as possible as far as I understand to codify the metrics to a certain degree because there's some aspects of it which is the lives in a group on a database. We can quantify the data migration for that, but it will probably be illegible to to have some of that data.} (P16)

% \q{T:it's growing and more stuff is getting codified. but other parts still you have to go in modify configuration or set something up manually. anyways} (P5)

% \q{T: right it's all the things you assume will happen but no one writes down. most NFRs are nice to haves and there are one or two that you have to have this, they are a design requirement that is like fixed but isn't necessarily codified. so I'd say for most NFRs they're usually not codified but that is something that DevOps is changing right? in terms of defining those. Do you want examples? like it's easier to find examples} (P5)

% \q{T: That's great thing actually what some of the devops stuff right is it if you can codify your alarm setup and it would just start to get flagged out. Definitely don't do that right now24:13} (P5)

% \q{T: Yeah, there's a piece of code. That's a script or whatever the runs all of that in terms of how the backups are running but there's pieces of it that probably aren't codified in terms of like from the terraform side of things. Like where is the bucket that the backups are sitting or where it's a region or like, how are the permissions managed on that? Some of that is codified and some isn't, like the process itself is codified in the sense that you that you take from here and put and you keep for this long. in terms of expires and things like that.} (P5)

% \q{T: Yeah, exactly. Yeah. We're not quite there on the PHP, but we're hoping to get there soon. I can't believe it took me a long time to think of that one. Yeah, yeah dependencies. They're all codified.} (P6)
%===============================================================================

